Relative Representations Enable Portable White-Box Monitoring Across Language Models

Independently trained autoregressive language models often acquire similar capabilities, but it remains unclear whether their internal representations organize behaviorally relevant information in compatible ways. We show that models do in fact organize information similarly by using specific behavioral probes that operate on compatible representations. This unlocks portable white-box monitoring: a probe developed and validated on one model can be reused when the model changes, without requiring labeled target data. To overcome incompatible native activation coordinates, we express each example through its angular distances to a shared set of anchors. We introduce a global anchored construction that summarizes information from all transformer layers and removes model-specific layer selection, so the same frozen probe can be straightforwardly applied to another model. We evaluate cross-model probe transfer across monitoring tasks on trivia datasets, safety monitoring, and mathematical reasoning. On average, transferred global anchored probes preserve at least 85% of same-model probe AUROC over chance. Anchored probes also support transfer to related datasets, remain robust across model scale and prompt changes, and retain performance better than standard probes after model updates. Transfer is nevertheless task- and target-dependent and can fail even when the monitored property remains strongly decodable in the target model. Overall, global anchoring reveals substantial task-relevant compatibility across independently trained models and provides a practical basis for portable white-box monitoring.

==> content/_tables/single_tables/guard/mlp/anchor_norm/agg-mean/anch600/params1_ls0.8/follow_up/baseline_guard-safety_recall.tex <==
% Generated by relative_probing/python_scripts/analysis/generate_guard_mlp_rebuttal_artifacts.py directly from saved Guard MLP and linear result JSONs.
\begin{table}[tbp]
\centering
\caption{Same-model Guard Distillation R@0.1FPR for linear and MLP probes with mean-token anchors. The MLP has 64 hidden units, and its global variant uses target-anchor normalization.}
\label{tab:guard-mlp-h64-baseline-recall}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccc}
\toprule
Dataset & Standard linear & Standard MLP & Global linear & Global MLP \\
\midrule
BeaverTails & $86.0\pm1.2$ & $80.7\pm1.6$ & $79.9\pm1.9$ & $78.3\pm2.5$ \\
Toxic-chat & $68.6\pm2.2$ & $58.4\pm2.4$ & $67.2\pm2.9$ & $51.9\pm0.5$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

